Uncertainties of Latent Representations in Computer Vision

Uncertainty quantification is a key pillar of trustworthy machine learning. It enables safe reactions under unsafe inputs, like predicting only when the machine learning model detects sufficient evidence, discarding anomalous data, or emitting warnings when an error is likely to be inbound. This is particularly crucial in safety-critical areas like medical image classification or self-driving cars. Despite the plethora of proposed uncertainty quantification methods achieving increasingly higher scores on performance benchmarks, uncertainty estimates are often shied away from in practice. Many machine learning projects start from pretrained latent representations that come without uncertainty estimates. Uncertainties would need to be trained by practitioners on their own, which is notoriously difficult and resource-intense. This thesis makes uncertainty estimates easily accessible by adding them to the latent representation vectors of pretrained computer vision models. Besides proposing approaches rooted in probability and decision theory, such as Monte-Carlo InfoNCE (MCInfoNCE) and loss prediction, we delve into both theoretical and empirical questions. We show that these unobservable uncertainties about unobservable latent representations are indeed provably correct. We also provide an uncertainty-aware representation learning (URL) benchmark to compare these unobservables against observable ground-truths. Finally, we compile our findings to pretrain lightweight representation uncertainties on large-scale computer vision models that transfer to unseen datasets in a zero-shot manner. Our findings do not only advance the current theoretical understanding of uncertainties over latent variables, but also facilitate the access to uncertainty quantification for future researchers inside and outside the field, enabling straightforward but trustworthy machine learning.

==> packages.tex <==
\usepackage[multiple]{footmisc}
\usepackage[eulermath,a5paper]{classicthesis_cw}
\usepackage[utf8x]{inputenc}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage[american]{babel}
\usepackage[T2A,T1]{fontenc}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{tcolorbox}
\usepackage{lettrine}
\usepackage{nameref}
\usepackage{natbib}
\renewcommand{\bibfont}{\fontsize{12}{14}\selectfont}
\setcitestyle{authoryear}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{afterpage}
\usepackage{xurl}
\usepackage{tikz}
\usetikzlibrary{positioning}
\usepackage[parfill]{parskip}
\usepackage{pdfpages}
\usepackage{listings}
\usepackage{inconsolata}
\usepackage[pdftex,pageanchor=true,bookmarks=true,bookmarksnumbered=true,backref=page,hyperindex=true]{hyperref}
\usepackage[tight]{minitoc}
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}


\RequirePackage[hyperpageref]{backref} 
   \renewcommand*{\backref}[1]{}  
   \renewcommand*{\backrefalt}[4]{
      \ifcase #1 
         %No cited.
      \or
         Cited on page #2.
      \else
         Cited on pages #2.
      \fi}

\definecolor{blue}{HTML}{4878D0}
\definecolor{red}{HTML}{D65F5F}
\definecolor{green}{HTML}{6ACC64}
\definecolor{orange}{HTML}{EE854A}
\definecolor{grey}{HTML}{797979}
\definecolor{lightgrey}{HTML}{adb3b7}
\definecolor{purple}{HTML}{7D3382}
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}

\lstset{
    backgroundcolor=\color{lightgray},
    basicstyle=\ttfamily,
    columns=fullflexible
}

\counterwithout{figure}{chapter}
\counterwithout{table}{chapter}

==> related_work.tex <==
\chapter{Related Work}
\label{chap:related}

\vspace*{-2.2em}
\minitoc
\vspace*{0.8em}

In this chapter, we review literature on ...
